Towards Computational Performance Engineering for Unsupervised Concept Drift Detection -- Complexities, Benchmarking, Performance Analysis

Concept drift detection is crucial for many AI systems to ensure the system's reliability. These systems often have to deal with large amounts of data or react in real-time. Thus, drift detectors must meet computational requirements or constraints with a comprehensive performance evaluation. However, so far, the focus of developing drift detectors is on inference quality, e.g. accuracy, but not on computational performance, such as runtime. Many of the previous works consider computational performance only as a secondary objective and do not have a benchmark for such evaluation. Hence, we propose and explain performance engineering for unsupervised concept drift detection that reflects on computational complexities, benchmarking, and performance analysis. We provide the computational complexities of existing unsupervised drift detectors and discuss why further computational performance investigations are required. Hence, we state and substantiate the aspects of a benchmark for unsupervised drift detection reflecting on inference quality and computational performance. Furthermore, we demonstrate performance analysis practices that have proven their effectiveness in High-Performance Computing, by tracing two drift detectors and displaying their performance data.

==> content/evaluation.tex <==
To show the necessity of thorough computational performance considerations, we conducted several experiments with four different drift detectors on four datasets.
%In this section, we show the necessity for computational performance considerations and explain the experiments we conducted with four different drift detectors on four datasets.
First, we introduce the relevant computational performance metrics that we measured. Second, we introduce the evaluated pipelines and \glspl{dd}, and present the datasets. Lastly, we show and discuss our experiment results. All experiments were performed five times and we report the average of the results. We also calculated the standard deviations but omitted them from the discussion as they were insignificant. 
All experiments were conducted on the HPC machine XXXXX at XXXXX.
We used a single CPU core of an AMD EPYC 7702 CPU, fixed to 2.0\,GHz frequency to improve reproducibility.
Since the implementations do not run in parallel, we do not consider multiple CPUs or nodes.
%All the experiments were conducted on an Intel i5-8265U CPU and 24GB memory.

\subsection{Metrics}
To assess the computational performance of a drift detector, we measure the overall runtime of the whole pipeline $R_{Sum}$ and the runtime of the drift detector $R_{DD}$. For $R_{Sum}$ we start the time measurement after loading the data and conducting an initial base model training. We end the measurement after processing the whole data stream.
For $R_{DD}$ we measure the time for everything, that is required to detect a drift and maintain the drift detector. We do not consider the drift handling, e.g. re-training of a base model, in case of a detected drift. Thus, we do not penalize a \gls{dd} for an expensive base model or drift handling strategy.
We can not compare $R_{Sum}$ or $R_{DD}$ across different approaches, since the default implementations are based on different programming languages and base models. Thus, we compute the Relative Runtime Overhead $RRO$ to compare the \glspl{dd} of the different pipelines as follows:
$$
RRO=\frac{R_{Sum}}{R_{Sum}-R_{DD}}
$$
Since the $RRO$ is a relative measure, we can compare it across different approaches. It gives a first measure for the runtime overhead that is introduced by the \gls{dd} in a pipeline.
We assess the $RRO$ w.r.t. the different approaches and the initially proposed base models and pipeline components to compare the runtime overhead. It is important to mention, that the $RRO$ is based only on the \gls{dd} and not on the overhead that is introduced by the continuous re-training of the model. 
However, a \gls{dd} triggers a drift handling method for each detected drift, e.g. model re-training. Thus, if a \gls{dd} is too sensitive, the runtime overhead for the whole pipeline will increase, due to the low inference quality of the \gls{dd}.
Thus, it is important to reflect on both 1) the computational performance and 2) the inference quality of a \gls{dd}. 
We also monitor the peak memory $M_{peak}$ of the overall pipeline with profilers for the individual programming languages.

For real-world datasets, it is difficult to compute the inference quality of a \gls{dd} directly, since the drift is always measured relative to a window of data samples that is maintained by the \gls{dd} itself. Furthermore, this would require further pre-investigation of the individual datasets.
Therefore, to reflect on the inference quality of the different \glspl{dd}, we measure the accuracy metric $Acc$ for the base \gls{ml} models of the different pipelines. Accuracy is determined by $Acc = \textit{correct decisions}/\textit{overall decisions}$.
Note that $Acc$ does not represent the proportion of correctly detected drifts. Instead, it indirectly reflects the inference quality of the \gls{dd}, since the accuracy of the \gls{ml} base model is affected by true and false drift detections. 
Since a detected drift always triggers a drift handling, that might cause additional computational overhead, we count the number of detected drifts as $Detections$. Moreover, since some of the related approaches request true labels after a detected drift, we monitor the relative amount of requested data labels with the $ReqLabels$ metric.

\subsection{Datasets}
For our experiments, we use five different real-world datasets as described in \autoref{table:datasets}.
The datasets Insects~\cite{souza2020challenges} and Abrupt Insects~\cite{souza2020challenges} consist of 50 dimensions with five different classes that refer to different insects. Abrupt Insects was shuffled in a way, that it consists of abrupt drift, i.e. the sudden change in the data distribution.
The UWave dataset~\cite{LiuUwave} consists of 4479 samples with 315 dimensions that represent accelerometer motion data of eight different gestures.
The Forest Covtype~\cite{blackard1999comparative} dataset consists of 54 features with seven different forest cover type designations. The data in KDDCUP99~\cite{misc_kdd_cup_1999_data_130} consists of 41 dimensions and each sample is assigned to either the Normal or Intrusion class.

For the datasets Insects, Abrupt Insects and UWave we use 500 labeled samples initially available for the training of a base \gls{ml} model. For the datasets Forest Covtype and KDDCUP99 we use 5000 labeled samples respectively. The rest of the data is used for the inference of the \gls{ml} model and our experiments w.r.t. concept drift detection and handling.

\begin{table}[t!]
		\caption{Datasets that were used for the evaluation.}
  \renewcommand{\arraystretch}{1.18}
\begin{tabular}{@{}b{0.5cm}@{}b{4.1cm}b{0.6cm}b{0.8cm}}
\multicolumn{1}{c}{\rotatebox{0}{Dataset}} & \multicolumn{1}{c}{\rotatebox{0}{Description}} & \multicolumn{1}{b{1.2cm}}{\rotatebox{0}{\makecell[lb]{Size}}} & \multicolumn{1}{b{0.8cm}}{\rotatebox{0}{Classes}} \\\hline
	Insects & Laser sensor data from flying insects & 5325x50 & 5\\\hline
    \makecell[lt]{Abrupt\\Insects} & The same as Insects, but shuffled to introduce abrupt drift& 5325x50 & 5\\\hline
    \makecell[lt]{UWave\\Gesture} & A set of eight gestures from accelerometers & 4479x315 & 8\\\hline
    \makecell[lt]{Forest\\Covtype} & Cartographic features to determine forest cover type& 581012x54 & 7\\\hline
    \makecell[lt]{KDD\\CUP99} & Network data containing intrusions and normal network traffic& $4.9*10^6$x41 & 2\\\hline
	\end{tabular}
	\label{table:datasets}
\end{table}

\iffalse
\begin{table}[t!]
		\caption{Datasets that were used for the evaluation.}
  \renewcommand{\arraystretch}{1.18}
\begin{tabular}{@{}b{0.5cm}@{}b{4.1cm}b{0.6cm}b{0.6cm}b{0.6cm}}
\multicolumn{1}{c}{\rotatebox{30}{Dataset}} & \multicolumn{1}{c}{\rotatebox{30}{Description}} & \multicolumn{1}{b{0.2cm}}{\rotatebox{30}{\makecell[lb]{\# Samples}}} & \multicolumn{1}{b{0.2cm}}{\rotatebox{30}{\# Dimensions}} & \multicolumn{1}{b{0.6cm}}{\rotatebox{30}{\# Classes}} \\\hline
	Insects & Laser sensor data from flying insects & 5325 & 50 & 5\\\hline
    \makecell[lt]{Abrupt\\Insects} & The same as Insects, but shuffled to introduce abrupt drift& 5325 & 50 & 5\\\hline
    \makecell[lt]{UWave\\Gesture} & A set of eight gestures from accelerometers & 4479 & 315 & 8\\\hline
    \makecell[lt]{Forest\\Covtype} & Cartographic features to determine forest cover type& 581012 & 54 & 7\\\hline
    \makecell[lt]{KDD\\CUP99} & Network data containing intrusions and normal network traffic& $4.9*10^6$ & 41 & 2\\\hline
	\end{tabular}
	\label{table:datasets}
\end{table}
\fi 
\subsection{Evaluated Drift Detectors}
From~\autoref{table:overviewDD}, six implementations are publicly available. We used the original Python implementations of \cite{dos2016fast} and \cite{cerqueira2022studd}, the original Java implementation of \cite{haque2016sand} and the original Matlab implementation of \cite{pinage2020drift}. 
We used the default pipelines of the approaches, but adapted some hyperparameters, following the guidance of the respective papers. Moreover, we made minor changes in the codebases in order to make the implementations run with the different datasets and for conducting our measurements. The code for our experiments will be available publicly~\footnote{\href{https://github.com/}{https://github.com/}}.
Note, for that initial investigation we skipped the implementations by Gözüaçık et al.~\cite{gozuaccik2019unsupervised, gozuaccik2021concept} since their pipelines conduct continual re-training of the \gls{ml} model with the true labels. Thus, even if their drift detection is fully unsupervised, they rely on the immediate availability of data labels across their whole pipeline and a comparison with the other methods requires adaptions of their pipelines.

\subsubsection{IKS}
The \gls{iks} was introduced by dos Reis et al.~\cite{dos2016fast} and detects drift based on the changes in the raw input data distribution. Therefore, it constructs a reference window and a detection window and compares the data distributions within these windows with a Kolmogorov-Smirnov test. The default implementation for \gls{iks} operates on a single input feature. In the case of drift, we follow the strategy of model replacement that was suggested in the original paper among other drift handling mechanisms. The model replacement strategy requests true labels and trains a new model. For our evaluation, we use a Random Forest with 100 decision trees as a base classifier.

\subsubsection{STUDD}
Cerqueira et al.~\cite{cerqueira2022studd} presented STUDD, an approach that follows a student-teacher learning paradigm. It consists of a student auxiliary model to mimic the behavior of a primary teacher decision model. Drift is detected if the mimicking loss of the student model changes w.r.t. the teacher's predictions. In case of a detected drift, the method updates the existing base model and student model with the requested true labels. As a basis for our evaluation, we use a Random Forest with 100 decision trees.

\subsubsection{SAND}
SAND is an approach for adapting and detecting novel classes over data streams and was introduced by Haque et al.~\cite{haque2016sand}. The classification is done by $K$-means clustering, setting the value of $K$ based on the size of the training data. Moreover, it consists of a concept drift detection that was introduced as \gls{bdcp} and operates on the confidences that \gls{ml} model emits in the
inference. \gls{bdcp} reports drift in case of drops in the confidences. In the original
paper, the authors recommend calling \gls{bdcp} in cases, where the confidences fall
under a certain threshold in order to reduce runtime. Therefore, we used
this procedure in our experiments. If a drift is detected, true labels are requested and the model is retrained.

\subsubsection{PinagéDD}
Pinagé et al~\cite{pinage2020drift} present DCS-LA+EDDM, a method that detects drift by monitoring the pseudo-error of an ensemble classifier. They use an ensemble of Hoeffding trees and select one of the ensemble members by DCS-LA~\cite{woods1997combination} method to provide the pseudo ground truth for unlabelled samples. The pseudo-error is then calculated w.r.t. this pseudo-ground truth. If the error changes, drift is detected and the ensemble is updated. DCS-LA+EDDM requires a training and a validation dataset for the internal pseudo-label generation. Therefore we separated the 500 samples into 350 samples training and 150 samples validation data for Abrupt Insects and Insects, 3500 and 1500 for Forest Covtype and KDDCUP99 respectively. Under the hood, DCS-LA+EDDM uses the supervised \gls{dd} EDDM~\cite{baena2006early} based on the pseudo-labels. In case of a detected drift, the pseudo-labels are used and no true labels are required. For ease of naming, we refer to DCS-LA+EDDM as PinagéDD.

Additionally, we measure two baselines that use a Random Forest with 100 decision trees as a classifier. Baseline1 does not conduct any re-training and Baseline2 updates the classifier after 500 samples for Insects, Abrupt Insects and UWave 5000 samples for Forest Covtype, and KDDCUP99 respectively. Both pipelines are implemented with Python. The setup is described and provided by~\cite{cerqueira2022studd} and supports the assessment of the \glspl{dd}' experiment results.


\begin{table}[t!]
		\caption{Evaluation of the approaches on the different datasets. $M_{Peak}$ is in Megabyte. A "-" for the baselines indicates, that there is no value for the metric available.}
  \renewcommand{\arraystretch}{1.18}
	\begin{tabular}{@{}b{1cm}@{\hspace{0.1cm}}b{1cm}b{0.4cm}b{0.4cm}b{0.5cm}b{0.7cm}b{0.7cm}b{0.4cm}b{0.4cm}} 
	%\hline
	\multicolumn{1}{@{}b{0.8cm}}{\rotatebox{30}{Dataset}} & \multicolumn{1}{@{}b{0.9cm}}{\rotatebox{30}{Approach}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$Accuracy$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$Detections$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$ReqLabels$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$R_{Sum}$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$R_{DD}$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$RRO$}} & \multicolumn{1}{@{}b{0.4cm}}{\rotatebox{30}{$M_{Peak}$}} \\\hline
	\multirow{4}*{Insects}
    & IKS & 78\% & 5 & 89\% & 34s & 5s & 1.17 & 189 \\\cline{2-9}
    & STUDD & 84\% & 0 & 0\% & 52s & 26s & 2.00 & 190  \\\cline{2-9}
    & SAND & 99\% & 4 & 77\% & 4s & 2s & 2.00 & 196 \\\cline{2-9}
    & PinagéDD & 78\% & 0 & 0\% & 143s & 48s & 1.50 & 629 \\\cline{2-9}
    & Baseline1 & 84\% & - & - & 25s & - & - & 185 \\\cline{2-9}
    & Baseline2 & 81\% & - & 100\% & 28s & - & - & 189 \\\hline
    \multirow{4}*{\makecell[lt]{Abrupt \\ Insects}}
    & IKS & 85\% & 6 & 34\% & 32s & 4s & 1.14 & 185 \\\cline{2-9}
    & STUDD & 83\% & 2 & 19\% & 57s & 30s & 2.11 & 193  \\\cline{2-9}
    & SAND & 98\% & 5 & 68\% & 17s & 15s & 8.5 & 230 \\\cline{2-9}
    & PinagéDD & 66\% & 1 & 0\% & 139s & 49s & 1.54 & 643 \\\cline{2-9}
    & Baseline1 & 65\% & - & - & 26s & - & - & 182 \\\cline{2-9}
    & Baseline2 & 79\% & - & 100\% & 29s & - & - & 187 \\\hline
    \multirow{4}*{\makecell[lt]{UWave \\ Gesture}}
    & IKS & 90\% & 0 & 0\% & 23s & 2s & 1.09 & 221 \\\cline{2-9} %only one feature, thus low overhead
    & STUDD & 90\% & 0 & 0\% & 43s & 21s & 1.95 & 223 \\\cline{2-9}
    & SAND & 80\% & 11 & 72\% & 8s & 2s & 1.33 & 211 \\\cline{2-9}
    & PinagéDD & 89\% & 0 & 0\% & 528s & 4s & 1.01 & 357\\\cline{2-9}
    & Baseline1 & 90\% & - & - & 21s & - & - & 222 \\\cline{2-9}
    & Baseline2 & 91\% & - & 100\% & 27s & - & - & 248 \\\hline
    \multirow{4}*{\makecell[lt]{Forest \\ Covtype}}
    & IKS & 85\% & 400 & 50\% & 5266s & 1138s & 1.27 & 704 \\\cline{2-9} 
    & STUDD & 68\% & 25 & 3\% & 10218s & 6108s & 2.48 &  1008 \\\cline{2-9}
    & SAND & 94\% & 1493 & 87\% & 5176s & 4910s & 20.15 & 388 \\\cline{2-9}
    & PinagéDD & 52\% & 8 & 0\% & 11970s & 3248s & 1.37 & 3756 \\\cline{2-9}
    & Baseline1 & 61\% & - & - & 4321s & - & - & 446 \\\cline{2-9}
    & Baseline2 & 80\% & - & 100\% & 4432s & - & - & 698 \\\hline
    \multirow{2}*{\makecell[lt]{KDD\\CUP99}}
    & \multicolumn{8}{c}{\multirow{2}{*}{no termination within 60min}}\\
    & \multicolumn{8}{c}{}\\\hline
   % \multirow{4}*{\makecell[lt]{Electric \\ Devices}}
   % & IKS & 45\% &  & 93\% & 199 & 47 &  &  \\\cline{2-9} 
   % & STUDD & 55\% & 3 & 9\% & 240 & 125 &  &  \\\cline{2-9}
   % & SAND & 54\% & 103 & 74\% &  & & & \\\cline{2-9}
   % & PinagéDD & & & & & & & \\\cline{2-9}
   % & Baseline1 & 56\% & - & - & 103 & - & - & \\\cline{2-9}
   % & Baseline2 & 51\% & - & 100\% & 109 & - & - & \\\hline
	\end{tabular}
	\label{table:earlyeval}
\end{table}


\subsection{Experiment Results}
\autoref{table:earlyeval} shows our experiment results.
We can see that the total absolute runtime of the approaches is high for all pipelines when dealing with the larger Forest Covtype dataset. For KDDCUP99, none of the approaches terminates within 60 minutes. However, we see differences in the runtimes, i.e. the Java implementation of SAND is always the fastest and the Matlab implementation of PinagéDD is always the slowest. 
Since it is difficult to compare these absolute runtimes, the $RRO$ provides a relative measure that reflects the overhead introduced by the drift detection.
It ranges from 1.09 to 1.27 for the \gls{iks}. For STUDD we measure higher runtime overheads, i.e. 1.95 - 2.48 due to drift detection. The reason for this is the expensive maintenance of the student model. 
Furthermore, each detected drift is followed by drift handling, which increases the total runtime $R_{Sum}$. Also for SAND the $RRO$ is high, i.e. 1.33-20.15, due to the fast inference times of the clustering base model and the relatively expensive computations for computing and maintaining the drift detection.
For PinagéDD the $RRO$ is lower, 1.01-1.54, because it uses a fast supervised \gls{dd} under the hood based on pseudo-true labels. However, creating these can be expensive and lead the model training in the wrong direction, as the pseudo-label could still be wrong.
Thus, PinagéDD does not require any true labels but has the lowest accuracy on average which can be even lower than Baseline1. The highest accuracy for all datasets, except UWave can be achieved with SAND. The reason for this could be the fast converging clustering model and the high amount of detected drift and requested true labels.
Next to PinagéDD, STUDD requires on average the least amount of labeled data. It still achieves good accuracy on the Insects and Abrupt Insects datasets but drops off on the Forest Covtype data. 
IKS detects a lot of drift and requests many data labels. However, IKS only operates on a single input feature, and varying the input feature under investigation could result in different behaviors. 
Memory consumption is insignificant for all pipelines.
In general, we observed a high sensitivity of all approaches to different hyperparameter settings. 
Thus, the interdependence of \glspl{dd}, their hyperparameters, base models, datasets and underlying hardware resources should be further investigated. In addition, other methods of drift handling, such as $\alpha/\beta$ transformation described in~\cite{dos2016fast}, could be investigated.
%Thus the runtime for \gls{iks} is higher than Baseline1 and even Baseline2 for Insects, Abrupt Insects and Forest Covtype. However, for UWave Gesture

\iffalse
The runtime for computing and maintaining the drift detection is reflected in the $RRO$ and ranges from 9\% to 27\% for the \gls{iks}. For STUDD we measure significantly higher runtime overheads, i.e. 99\% - 147\% due to drift detection. The reason for this is the expensive maintenance of the student model. 
Furthermore, each detected drift is followed by drift handling, which increases the total runtime $R_{Sum}$. Thus the runtime for \gls{iks} is higher than Baseline1 and even Baseline2 for the small datasets.
SAND has the lowest runtime and highest accuracy for all datasets, except UWave. The reason for this might be the implementation in Java and the fast-converging clustering model. However, it requests many labels and the $RRO$ is high for all experiments.
For PinagéDD the $RRO$ is lower, about 5\%, because it uses a fast supervised \gls{dd} under the hood. However, the creation of the required pseudo-true label can be expensive and can lead the model training in the wrong direction when processing the data, as the pseudo-label could still be wrong.
Next to PinagéDD, STUDD requires on average the least amount of labeled data. It still achieves good accuracy on the Insects and Abrupt Insects datasets but falls off on the Forest Covtype data. IKS and SAND request a lot of labels, as both approaches detect a lot of drift.
However, IKS only operates on a single input feature, and varying the input feature under investigation could lead to different behaviors. In general, we observed high sensitivities of all approaches for different hyperparameter settings. 
%We decided to present the results based on the best hyperparameter we could achieve.
Therefore, the interdependence of \glspl{dd}, their hyperparameters and base models, datasets and underlying hardware resources can be further investigated. In addition, other methods of drift handling, such as the $\alpha/\beta$ transformation described in~\cite{dos2016fast}, which do not require true labels, could be investigated.
Memory consumption is highest for STUDD. However, it can be considered insignificant for all pipelines.
\fi


\subsection{Discussion}

%Especially for larger datasets we observe high pipeline runtimes. One component that increases the runtime of these pipelines is the \gls{dd}, which affects the overall runtime through its own computations, but also through the drift handling that is triggered after a drift is detected.

As demonstrated in the experiments, concept drift detection can be an important pillar to guarantee the robustness of AI applications. Without proper drift detection, the accuracy of the pipelines would decrease significantly as shown by Baseline1. Also, as Baseline2 shows, a pure re-training approach might not help to maintain the robustness of a \gls{ml} application and might increase the runtime of the whole pipeline.
However, from the publicly available approaches, there is no unsupervised \gls{dd} available that fulfills the need for high detection accuracy, without many required true labels while having a low runtime overhead. A comprehensive benchmark of unsupervised \glspl{dd} is not yet available but is required to assess the behavior of available \glspl{dd} and to identify strengths and bottlenecks in current approaches.
\iffalse
For drift detection, computational performance and inference quality may be interrelated and depend on the data, parameters of the \gls{dd} and the base \gls{ml} model in the pipeline, e.g. a \gls{dd} that detects a high number of drift always causes higher runtimes due to the triggered drift handling. Furthermore, as outlined in \autoref{table:overviewDD}, some \glspl{dd} operate on the pure input data, while others require the confidence or error rates of the base \gls{ml} model.
Thus, the benchmarking has to consider many different base classifiers and hyperparameter settings in order to obtain representative results for a comprehensive comparison between different \glspl{dd}.
Since the experimental space would be huge in this case, an alternative would be to simulate the output of a \gls{ml} model. It would then be possible to investigate different \glspl{dd} w.r.t. requirements of a \gls{ml} model in terms of its inference quality. This would allow more specific investigations of \gls{dd} and \gls{ml} model combinations in an AI pipeline.

In addition, benchmarks should be conducted based on different datasets from real-world domains and synthetic sources. While real-world data provide insight into the behaviour in real-world applications, synthetic datasets are helpful to test specific characteristics by defining patterns of concept drift in advance. In addition, it may be interesting to investigate the effect of data size per sample point, which can be further reflected in experiments with different datasets. 

The benchmark also needs to consider various evaluation metrics representing aspects of computational performance and inference quality. We have proposed an initial set of metrics to support the investigations. However, although the $RRO$ provides an initial measure to compare different approaches across implementations, a fair comparison requires further steps. We need proper implementations using the same programming language. Implementations should be publicly available for the majority of approaches and should be extensively documented. We also need theoretical considerations of the time and memory complexity of the approaches and compare them. 
We should also aim for scalable and parallel solutions for drift detection. A first approach was presented in~\cite{grulich2018scalable}, where a parallel implementation of the supervised \gls{dd} ADWIN~\cite{grulich2018scalable}.
\fi
Hence, we propose to consider the following aspects when conducting a benchmark for unsupervised \glspl{dd}.
\subsubsection{Metrics}
For drift detection, computational performance and inference quality are interrelated and depend on the data, the parameters of the \gls{dd} and the base \gls{ml} model in the pipeline, e.g. a \gls{dd} that detects a high number of drift causes higher runtimes due to triggered drift handling.
Therefore, the whole landscape of unsupervised \glspl{dd} should be investigated from both perspectives: inference quality and computational performance. We proposed a first set of metrics to support this investigation. However, although the $RRO$ provides an initial measure to compare different approaches across implementations, a fair comparison requires further steps.

\subsubsection{Implementation and Methodology}
We need proper implementations with the same programming language in order to make approaches comparable. Implementations should be publicly available and should be extensively documented. We also need theoretical considerations of the time and memory complexity of the approaches, and comparisons between them.
Furthermore, as outlined in \autoref{table:overviewDD}, some \glspl{dd} operate on the pure input data, while others require the confidence or error rates of the base \gls{ml} model.
Thus, the benchmarking has to consider many different base classifiers and hyperparameter settings in order to obtain representative results for a comprehensive comparison between different \glspl{dd}.
Since the experimental space would be huge in this case, an alternative would be to simulate the output of a \gls{ml} model. It would then be possible to investigate different \glspl{dd} w.r.t. requirements of a \gls{ml} model and its inference quality. This would allow more specific investigations of \gls{dd} and \gls{ml} model combinations in an AI pipeline.

\subsubsection{Datasets}
In addition, benchmarks should be conducted based on different datasets from real-world domains and synthetic sources. While real-world data provide insights into the behavior in real applications, synthetic datasets are helpful in testing specific characteristics by defining patterns of concept drift in advance. In addition, it may be interesting to investigate the effect of data size per sample point, which can be reflected in experiments with various datasets. 

Thus, a comprehensive benchmark supports the community in assessing available approaches and helps to develop novel solutions, including parallel and scalable implementations as proposed by Grulich et al. for the supervised \gls{dd} ADWIN~\cite{grulich2018scalable}.
